Open system control of dynamical transitions under the generalized Kruskal-Neishtadt-Henrard theorem

Useful dynamical processes often begin through barrier-crossing dynamical transitions; engineering system dynamics in order to make such transitions reliably is therefore an important task for biological or artificial microscopic machinery. Here we first show by example that adding even a small amount of back-reaction to a control parameter, so that it responds to the system's evolution, can significantly increase the fraction of trajectories that cross a separatrix. We then explain how a post-adiabatic theorem due to Neishtadt can quantitatively describe this kind of enhancement without having to solve the equations of motion, allowing systematic understanding and design of a class of self-controlling dynamical systems.

==> images/SepaChute.tex <==


\begin{tikzpicture}[
%We set the scale and define some styles
%scale=\tikzscale,
axis/.style={very thick, ->, >=stealth'},
important line/.style={thick},
dashed line/.style={dashed, thick},
every node/.style={color=black,}
]
% Important coordinates are defined
%\coordinate (beg_1) at (0,-.5);
%\coordinate (beg_2) at ($(beg_1)+(1,0)$);
%\coordinate (dev_1) at ($(beg_2)+(0,-.75)$);
%\coordinate (xint) at (4,0);
%\coordinate (end) at (5,1.25);



\begin{scope}[every node/.append style={
	yslant=0.2,xslant=0},yslant=0.2,xslant=0
]
\coordinate (IpL1) at (0,2.5);
\coordinate (IpR1) at (5,2.5);
\coordinate (Im1) at (2.5,2.5);

\coordinate (R21) at (0,5);


\coordinate (G11) at (1,0);
\coordinate (G21) at (5,0);
\coordinate (G31) at (5,4);

\coordinate (LU1) at (0,0);
\coordinate (LO1) at (0,5);
\coordinate (RO1) at (5,5);
\coordinate (RU1) at (5,0);
\draw (IpR1) to [out=90, in=45]  (IpL1) 	;
\draw (IpR1) to [out=-90, in=-45] (IpL1) 	;

\draw[axis] (LU1)  -- (G21); %node[right] {$J$};
\draw (LU1)  -- (G21) node[midway,below] {$q$};

\draw[axis] (LU1) -- (R21); %node[above] {$I$};
\draw (LU1) -- (R21) node[midway,left] {$p$}    ;
\end{scope}

\begin{scope}[yshift=-85,xshift=100,every node/.append style={
	yslant=0.2,xslant=0},yslant=0.2,xslant=0
]
\coordinate (IpL2) at (0,2.5);
\coordinate (IpR2) at (5,2.5);
\coordinate (Im2) at (2.5,2.5);

\coordinate (R22) at (0,5);


\coordinate (G12) at (1,0);
\coordinate (G22) at (5,0);
\coordinate (G32) at (5,4);

\coordinate (LU2) at (0,0);
\coordinate (LO2) at (0,5);
\coordinate (RO2) at (5,5);
\coordinate (RU2) at (5,0);
\shade[bottom color=orange, top color=orange]
(IpR2) to [out=90, in=45] (IpL2) to [out=-45, in=-90] (IpR2); 
\draw(IpR2) to [out=90, in=45]  (IpL2) 	;
\draw (IpR2) to [out=-90, in=-45] (IpL2) 	;
\node at (2.5,2.5) {$A(\lambda)$} ;
\end{scope}

\draw (LU1) -- (LU2) node[midway,left,below] {$\lambda$}    ;
\draw[axis] (LU1) -- (LU2);
% axis
\draw (IpR2) -- (IpR1) ;
\draw (IpL2) -- (IpL1) ;
\node at (IpR2) {$\qquad$} ;
%\draw (x2) -- (x1) ;
%\draw (y2) -- (y1) ;
%\draw[black,fill=black] (Im) circle (.05) node[right] {$I_-$};

%\draw[black,fill=black] (IpL) circle (.05) ;  
%\draw[dashed] (IpL) -- (IpR) node[midway,below] {$I_-$} ;

\end{tikzpicture}

==> images/Setup.tex <==
\begin{tikzpicture}[
	%We set the scale and define some styles
	%scale=\tikzscale,
	axis/.style={very thick, ->, >=stealth'},
	important line/.style={thick},
	dashed line/.style={dashed, thick},
	every node/.style={color=black,}
	]
	% Important coordinates are defined
	%\coordinate (beg_1) at (0,-.5);
	%\coordinate (beg_2) at ($(beg_1)+(1,0)$);
	%\coordinate (dev_1) at ($(beg_2)+(0,-.75)$);
	%\coordinate (xint) at (4,0);
	%\coordinate (end) at (5,1.25);
	
	\begin{scope}[yshift=-85,xshift=100,every node/.append style={
			yslant=0,xslant=0},yslant=0,xslant=0
		]
		\coordinate (IpL2) at (0,2.5);
		\coordinate (IpR2) at (5,2.5);
		\coordinate (Im2) at (2.5,2.5);
		\coordinate (R22) at (0,5);
		
		\coordinate (IpL1) at (0,2.5);
		\coordinate (IpR1) at (-3,2.5);
		
		
		\coordinate (G12) at (1,0);
		\coordinate (G22) at (5,0);
		\coordinate (G32) at (5,4);
		
		\coordinate (LU2) at (0,0);
		\coordinate (LO2) at (0,5);
		\coordinate (RO2) at (5,5);
		\coordinate (RU2) at (5,0);
		
		\shade[bottom color=orange, top color=orange]
		(IpR2) to [out=90, in=45] (IpL2) to [out=-45, in=-90] (IpR2); 
		\draw(IpR2) to [out=90, in=45]  (IpL2) 	;
		\draw (IpR2) to [out=-90, in=-45] (IpL2) 	;
		\node at (2.5,2.5) {$A_2$} ;
		
			\shade[bottom color=blue, top color=cyan]
		(IpR1) to [out=90, in=135] (IpL1) to [out=-135, in=-90] (IpR1); 
		\draw(IpR1) to [out=90, in=135]  (IpL1) 	;
		\draw (IpR1) to [out=-90, in=-135] (IpL1) 	;
		\node at (-1.5,2.5) {$A_1$} ;
		
		\node at (-0.5,3.5) {$D_0$} ;
	\end{scope}
	
	%\draw (x2) -- (x1) ;
	%\draw (y2) -- (y1) ;
	%\draw[black,fill=black] (Im) circle (.05) node[right] {$I_-$};
	
	%\draw[black,fill=black] (IpL) circle (.05) ;  
	%\draw[dashed] (IpL) -- (IpR) node[midway,below] {$I_-$} ;
	
\end{tikzpicture}
